Do Large Language Models Need a Content Delivery Network?

As the use of large language models (LLMs) expands rapidly, so does the range of knowledge needed to supplement various LLM queries. Thus, enabling flexible and efficient injection of new knowledge in LLM inference is critical. Three high-level options exist: (i) embedding the knowledge in LLM's weights (i.e., fine-tuning), (ii) including the knowledge as a part of LLM's text input (i.e., in-context learning), or (iii) injecting the KV caches of the new knowledge to LLM during prefill. This paper argues that, although fine-tuning and in-context learning are popular, using KV caches as the medium of knowledge could simultaneously enable more modular management of knowledge injection and more efficient LLM serving with low cost and fast response. To realize these benefits, we envision a Knowledge Delivery Network (KDN), a new system component in LLM services that dynamically optimizes the storage, transfer, and composition of KV cache across LLM engines and other compute and storage resources. We believe that, just like content delivery networks (CDNs), such as Akamai, enabled the success of the Internet ecosystem through their efficient data delivery, KDNs will be critical to the success of LLM applications through their efficient knowledge delivery. We have open-sourced a KDN prototype at https://github.com/LMCache/LMCache.

==> abstract_v2_deprecated.tex <==
\begin{abstract}

As the use of large language models (LLMs) expands rapidly, so does the range of knowledge needed to supplement various LLM queries in the real world.
% to generate high-quality responses. 
Thus, a crucial question is how LLMs learn new knowledge not seen during LLM's training. 
%Three high-level options exist: % to embed new knowledge:  
Two popular options exist:
{\em (i)} LLM's weights (\ie fine-tuning), or
{\em (ii)} a part of LLM's input (\ie in-context learning).
%{\em (iii)} KV caches loaded in GPU memory. 
This short paper argues {\em KV caches, as an alternate medium of new knowledge, could potentially be more manageable, more cost-efficient, and achieve better user experience.}
To realize such potential, we propose {\em Knowledge Delivery Networks (KDNs)}, a new system component to store, merge, and distribute knowledge as KV caches.
%, if they are managed by a new system component, we referred to as {\em Knowledge Delivery Networks} (KDNs)}.
We believe that, just like Content Delivery Networks (CDNs) like Akamai enabled most web applications, a KDN will be key to the success of LLM applications. 

\end{abstract}

==> existing_solution.tex <==
\section{Managing Knowledge for LLMs}

% Two solutions
In LLM applications, in-context learning and fine-tuning are two primary methods employed to incorporate new knowledge. 
In-context learning refers to the ability of an LLM to understand and generate responses based on the context provided in the prompt without altering the model's parameters. 
It leverages the existing capabilities of the model to interpret and respond to new information dynamically. 
On the other hand, fine-tuning involves retraining the model on a new dataset with specific tasks or knowledge, thereby updating its parameters to improve its performance on those tasks. 
Fine-tuning adjusts the internal parameters of the model to better capture the nuances of the new knowledge in the dataset.

Examples of both in-context learning and fine-tuning are abundant. 
For instance, in-context learning is used when an LLM is given a few text segments that contain useful background knowledge (\eg several sentences demonstrating a particular style or topic) to generate appropriate responses. 
This method is useful for applications requiring immediate adaptation to specific contexts, such as customer service chatbots or creative writing aids. 
Conversely, fine-tuning is used in scenarios where a model is retrained on specialized datasets to enhance its performance in a specific domain, like medical diagnosis or legal document analysis. 

% AI perspective
The AI research has a long literature on the pros and cons of in-context learning and fine-tuning. 
In-context learning can enhance quality by allowing users to control the input context, thereby reducing hallucinations and increasing coherence in the model's responses. 
This method excels when the new knowledge is specific and can be encapsulated within the provided context~\cite{??,??}. 
Fine-tuning tends to yield better results when integrating new knowledge across a large corpus of data. 
By updating the model's parameters, fine-tuning can ensure a deeper and more comprehensive understanding of the new information, leading to more accurate output in some cases~\cite{??,??}.

% Differently, we want to compare from system perspective. 
In contrast to the AI-centric view, which mainly evaluates the generation quality by accuracy or F1 score, we compare the solutions on the dimensions from the system perspective.
The first dimension is modularity, which means whether the approach supports swapping knowledge without affecting other components in the system.
The second dimension is response delay, defined by the time it takes from LLM receiving the user's input to the generation of the first token.

In-context learning is a modular design, since swapping knowledge can be done by simply changing the input context.
Such modular design offers multiple benefits. 
Firstly, it allows operators (\ie service providers) to control which knowledge to use.
In the real world, different knowledge may conflict with each other. 
For instance, different model providers may claim their model is better than others. \yh{think about a better example here}
Having explicit control of the knowledge helps the operator avoid such conflicts and improve the quality of the LLM's response.
Secondly, hundreds of websites are created every minute~\cite{??}, and in-context learning 
 can incorporate such new knowledge without extra overhead. 
In contrast, fine-tuning is not modular, because it puts all the knowledge in the model weights.
In this case, the operators cannot control the knowledge used to generate the answer and putting all knowledge into one model dilutes its ability to perform well in domain-specific tasks~\cite{??}. 
Also, fine-tuning needs to happen for every new knowledge and new model, and takes hours to days to complete.

On the other hand, in-context learning increases the response delay, because it needs to {\em prefill} the longer input text with knowledge before generating the first token.
In the prefill phase, the LLM takes in the input tokens, runs the attention operation, and gets the KV cache tensor for future token generation.
In all mainstream LLMs, the time for attention operation grows superlinearly with the input length.
In practice, the overhead of prefilling a 12-page paper is XXX seconds when using XXX model.
Fine-tuning has already embedded the knowledge in the model weights, so it only needs a short input and can avoid the overhead of prefilling long texts.

In short, Figure~\ref{??} compares in-context learning and fine-tuning from the system perspective. In-context learning is more modular but sacrifices the response delay, while fine-tuning, as a non-modular design, can generate the response with a lower delay.



==> existing_solution_v2.tex <==
 
\begin{figure*}[t!]
    \centering
    \hspace*{-0.35cm}\includegraphics[width=1.92\columnwidth]{figs/comparison-v2.pdf}
    \tightcaption{(Placeholder) Comparison between different solutions\jc{this will be replaced with a table}}
    \label{fig:comparison}
\end{figure*}

% \section{Managing Knowledge for LLMs}
% \section{How to inject new knowledge to LLMs}
\section{System Tradeoffs of Knowledge Injection in LLMs}

\jc{let's have a diagram contrasting the embedding knowledge INSIDE the model (fine-tuning) vs. SEPARATING the knowledge from the model (in-context and kv cache learning)}

% Two solutions
\begin{comment}
\jc{the following two paragraphs should be in the background, right?}
Traditionally, in-context learning and fine-tuning are the two popular knowledge-injection methods employed by LLM applications that require new knowledge. 
% In LLM applications, in-context learning and fine-tuning are two primary methods employed to incorporate new knowledge. 
In-context learning refers to the ability of an LLM to understand and generate responses based on the context provided as part of the prompt without altering the model's parameters. 
It leverages the existing capabilities of the model to interpret and respond to new information dynamically. 
On the other hand, fine-tuning involves retraining the model on a new dataset with specific tasks or knowledge, thereby updating its parameters to improve its performance on those tasks. 
Fine-tuning adjusts the internal parameters of the model to better capture the nuances of the new knowledge in the dataset.

Examples of both in-context learning and fine-tuning are abundant. 
For instance, in-context learning is used when an LLM is given a few text segments that contain useful background knowledge (\eg several sentences demonstrating a particular style or topic) to generate appropriate responses. 
This method is useful for applications requiring immediate adaptation to specific contexts, such as customer service chatbots or creative writing aids. 
Fine-tuning, on the other hand, retrains a model on a specialized dataset to enhance its performance in a specific domain, like medical diagnosis or legal document analysis. 
\end{comment}

% AI perspective
The AI research has a long literature on the pros and cons of in-context learning and fine-tuning. 
In-context learning can enhance quality by allowing users to control the input context, thereby reducing hallucinations and increasing coherence in the model's responses. 
This method excels when the new knowledge is specific and can be encapsulated within the provided context~\cite{??,??}. 
Fine-tuning tends to yield better results when integrating new knowledge across a large corpus of data. 
By updating the model's parameters, fine-tuning can ensure a deeper and more comprehensive understanding of the new information, leading to more accurate output in some cases~\cite{??,??}.

% Differently, we want to compare from system perspective. 
Instead of viewing these options only in terms of accuracy (\ie through the ML perspective), 
% In contrast to the AI-centric view, which mainly evaluates the generation quality by accuracy or F1 score, 
we compare these knowledge-injection methods along the following two dimensions from the system perspective: {\em modularity} and {\em performance}
\begin{itemize}
\item The {\em modularity} of a knowledge-injection method includes two aspects. Composability and evolvability
\item The {\em performance} of a knowledge-injection method includes two aspects. 
%\item The {\em modularity} of a knowledge-injection method means whether the approach supports flexibly specifying and changing the knowledge.
%\item {\em Cost efficiency} measures how much cost, in computation, storage, and communication, is needed for the LLM to incorporate the new knowledge.
%\item {\em Response delay} is defined by the time it takes from receiving the user's input that requires some new knowledge unseen by the original LLM to the generation of the first token.
\end{itemize}

% {\em modularity}, {\em cost efficiency}, and {\em fast response}.

% without causing side effects to other system components.





% \begin{figure}
%     \centering
%     \hspace*{-0.35cm}\includegraphics[width=.92\columnwidth]{figs/placeholder-figure-comparison.pdf}
%     \tightcaption{(Placeholder) Comparison between different solutions}
%     \label{fig:comparison}
% \end{figure}

%The first dimension is modularity, which means whether the approach supports flexibly specifying and changing knowledge without causing side effects to other components in the system.
As shown in Figure~\ref{fig:comparison} in-context learning is more modular since changing knowledge can be done by simply altering the input context.
Such modular design offers multiple benefits. 
Firstly, in-context learning allows operators (\ie service providers) to control which knowledge to use.
%In the real world, different knowledge may conflict with each other. 
%For instance, different model providers may claim their model is better than others. \yh{think about a better example here}
Having explicit control of the knowledge helps the operator avoid conflicting knowledge and improves the quality of the LLM's response. \yh{Example?}
However, in-context learning has considerable overhead in both cost and response delay. 
This is because LLMs need to {\em prefill} the longer input text with knowledge before generating the first token.
In the prefilling, the LLM takes in the input tokens, runs the attention operation, and gets the KV cache tensor for future token generation.
In all mainstream LLMs, the time for attention operation grows superlinearly with the input length.
In practice, the overhead of prefilling a 12-page paper is XXX seconds~\cite{??}\footnote{With XXX model and XXX GPU}.
Even if the knowledge is reused across different requests, in-context learning still needs to redo the prefill, leading to extra overheads in cost and response delay.

%Secondly, hundreds of websites are created every minute~\cite{??}, and in-context learning 
% can incorporate such new knowledge without extra overhead. 
%In contrast, fine-tuning is not modular, because it puts all the knowledge in the model weights.
%In this case, the operators cannot control the knowledge used to generate the answer, and putting all knowledge into one model dilutes its ability to perform well in domain-specific tasks~\cite{??}. 
On the other hand, fine-tuning can skip prefilling the long input, because the knowledge has already been embedded in the model weights and thus the input text can be short.
However, it suffers from modularity and cost dimensions.
First, service providers cannot control the knowledge used to generate the answer, and putting all knowledge into one model dilutes its ability to perform well in domain-specific tasks~\cite{??}. 
Moreover, fine-tuning needs to happen for every new knowledge and model, which may take hours to days to complete.

%The second dimension is response delay, which is defined by the time it takes from LLM receiving the user's input to the generation of the first token.
%In-context learning increases the response delay, because it needs to {\em prefill} the longer input text with knowledge before generating the first token.
%In the prefill phase, the LLM takes in the input tokens, runs the attention operation, and gets the KV cache tensor for future token generation.
%In all mainstream LLMs, the time for attention operation grows superlinearly with the input length.
%In practice, the overhead of prefilling a 12-page paper is XXX seconds when using XXX model.
%Fine-tuning has already embedded the knowledge in the model weights, so it only needs a short input and can avoid the overhead of prefilling long texts.

%In short, Figure~\ref{??} compares in-context learning and fine-tuning from the system perspective. In-context learning is more modular but sacrifices the response delay, while fine-tuning, as a non-modular design, can generate the response with a lower delay. \yh{add a few words about cost}

In short, as shown in Figure~\ref{fig:comparison}, in-context learning is more modular but sacrifices the cost-efficiency response delay, while fine-tuning, though achieving a lower response delay, suffers from bad modularity and the high cost of incorporating new knowledge.


==> existing_solution_v3.tex <==
%\begin{figure*}[t!]
%    \centering
%    \hspace*{-0.35cm}\includegraphics[width=1.92\columnwidth]{figs/comparison-v2.pdf}
%    \tightcaption{(Placeholder) Comparison between different solutions\jc{this will be replaced with a table}}
%    \label{fig:comparison}
%\end{figure*}



% \section{Managing Knowledge for LLMs}
% \section{How to inject new knowledge to LLMs}
% \vspace{-6pt}
\section{System Tradeoffs of Knowledge Injection in LLMs}
\label{sec:tradeoffs}

%\jc{let's have a diagram contrasting the embedding knowledge INSIDE the model (fine-tuning) vs. SEPARATING the knowledge from the model (in-context and kv cache learning)}

% Two solutions
\begin{comment}
\jc{the following two paragraphs should be in the background, right?}
Traditionally, in-context learning and fine-tuning are the two popular knowledge-injection methods employed by LLM applications that require new knowledge. 
% In LLM applications, in-context learning and fine-tuning are two primary methods employed to incorporate new knowledge. 
In-context learning refers to the ability of an LLM to understand and generate responses based on the context provided as part of the prompt without altering the model's parameters. 
It leverages the existing capabilities of the model to interpret and respond to new information dynamically. 
On the other hand, fine-tuning involves retraining the model on a new dataset with specific tasks or knowledge, thereby updating its parameters to improve its performance on those tasks. 
Fine-tuning adjusts the internal parameters of the model to better capture the nuances of the new knowledge in the dataset.

Examples of both in-context learning and fine-tuning are abundant. 
For instance, in-context learning is used when an LLM is given a few text segments that contain useful background knowledge (\eg several sentences demonstrating a particular style or topic) to generate appropriate responses. 
This method is useful for applications requiring immediate adaptation to specific contexts, such as customer service chatbots or creative writing aids. 
Fine-tuning, on the other hand, retrains a model on a specialized dataset to enhance its performance in a specific domain, like medical diagnosis or legal document analysis. 
\end{comment}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.94\linewidth]{figs/inside-and-outside.pdf}
%    \tightcaption{Different knowledge-injection methods put the knowledge in different places, leading to different modularity and efficiency.}
%    \label{fig:knowledge-placing}
%\end{figure}

% AI perspective
The AI research has a long literature studying in-context learning and fine-tuning. 
In-context learning can enhance quality by allowing users to control the input context, thereby reducing hallucinations and increasing coherence in the model's responses. 
%This method excels when the new knowledge is specific and can be encapsulated within the provided context~\cite{??,??}. 
Fine-tuning tends to yield better results when integrating new knowledge across a large corpus of data. 
%By updating the model's parameters, fine-tuning can ensure a deeper and more comprehensive understanding of the new information, leading to more accurate output in some cases~\cite{??,??}. \yh{remember to cite the raft paper}
Both methods can achieve similar text-generation quality if used in the right way~\cite{gupta2024rag, zhang2024raft, alghisi2024should}.

% Differently, we want to compare from system perspective. 
Instead of viewing these options only in terms of accuracy (\ie through the ML perspective), 
% In contrast to the AI-centric view, which mainly evaluates the generation quality by accuracy or F1 score, 
we compare the knowledge-injection methods along the following two dimensions from a system perspective: {\bf modularity} and {\bf efficiency}.

%The {\em modularity} of a knowledge-injection method includes two aspects. 
The {\em modularity} includes two aspects. 
First, a modular approach should allow service providers to specify which knowledge to use and compose them easily.
%support flexibly specifying and composing the existing knowledge during the inference.
Second, the overhead (\eg time, cost) of injecting new knowledge into the LLM should be minimized. % in a modular approach.

The {\em efficiency} is measured by per-query cost and response delay during LLM inference.
Cost is the computation used for the LLM to handle a request, and response delay is defined as the time between the LLM receiving the request and the generation of the first token.
%\begin{itemize}
%\item The {\em modularity} of a knowledge-injection method includes com
%\item The {\em performance} of a knowledge-injection method includes two aspects. runtime cost and performance
%%\item The {\em modularity} of a knowledge-injection method means whether the approach supports flexibly specifying and changing the knowledge.
%%\item {\em Cost efficiency} measures how much cost, in computation, storage, and communication, is needed for the LLM to incorporate the new knowledge.
%%\item {\em Response delay} is defined by the time it takes from receiving the user's input that requires some new knowledge unseen by the original LLM to the generation of the first token.
%\end{itemize}

% {\em modularity}, {\em cost efficiency}, and {\em fast response}.

% without causing side effects to other system components.





% \begin{figure}
%     \centering
%     \hspace*{-0.35cm}\includegraphics[width=.92\columnwidth]{figs/placeholder-figure-comparison.pdf}
%     \tightcaption{(Placeholder) Comparison between different solutions}
%     \label{fig:comparison}
% \end{figure}

%Figure~\ref{fig:comparison} compares the knowledge-injection solutions from the above two dimensions.
%As shown in Figure~\ref{fig:knowledge-placing}(a), 
In-context learning puts the knowledge in the model's input, making it easier to incorporate new knowledge and compose different ones. 
The separation of knowledge and model ensures enhanced modularity --- LLM service providers can clearly specify which knowledge to use and easily compose different pieces of knowledge, helping LLM avoid conflicting knowledge and improve the generation quality.
However, in-context learning has considerable runtime overhead that hurts efficiency. 
Specifically, when using in-context learning, LLMs must {\em prefill} a long input text with the knowledge before generating the first token.
%During the prefill, the LLM takes in the input tokens, runs the attention operation, and gets the KV cache tensor for future token generation.
During the prefill, the LLM takes in the input text and runs the attention operation, whose complexity grows superlinearly with the input length in all mainstream LLMs.
In many use cases, the prefill may block the GPUs up to tens of seconds~\cite{zhong2024distserve, cachegen}, leading to high GPU cost and long response delay.
%In all mainstream LLMs, the complexity for attention operation grows superlinearly with the input length, and each prefill may block the GPUs up to tens of seconds~\cite{zhong2024distserve, cachegen} in many use cases.
%In practice, the overhead of prefilling a 12-page paper is XXX seconds~\cite{??}\footnote{With XXX model and XXX GPU}.
%Even if the knowledge is reused across different requests, in-context learning still needs to redo the prefill, leading to extra overheads in cost and response delay.

%The first dimension is modularity, which means whether the approach supports flexibly specifying and changing knowledge without causing side effects to other components in the system.
%As shown in Figure~\ref{fig:comparison} in-context learning is more modular since changing knowledge can be done by simply altering the input context.
%Such modular design offers multiple benefits. 
%Firstly, in-context learning allows operators (\ie service providers) to control which knowledge to use.
%In the real world, different knowledge may conflict with each other. 
%For instance, different model providers may claim their model is better than others. \yh{think about a better example here}
%Having explicit control of the knowledge helps the operator avoid conflicting knowledge and improves the quality of the LLM's response. \yh{Example?}
%However, in-context learning has considerable overhead in both cost and response delay. 
%This is because LLMs need to {\em prefill} the longer input text with knowledge before generating the first token.
%In the prefilling, the LLM takes in the input tokens, runs the attention operation, and gets the KV cache tensor for future token generation.
%In all mainstream LLMs, the time for attention operation grows superlinearly with the input length.
%In practice, the overhead of prefilling a 12-page paper is XXX seconds~\cite{??}\footnote{With XXX model and XXX GPU}.
%Even if the knowledge is reused across different requests, in-context learning still needs to redo the prefill, leading to extra overheads in cost and response delay.

%Secondly, hundreds of websites are created every minute~\cite{??}, and in-context learning 
% can incorporate such new knowledge without extra overhead. 
%In contrast, fine-tuning is not modular, because it puts all the knowledge in the model weights.
%In this case, the operators cannot control the knowledge used to generate the answer, and putting all knowledge into one model dilutes its ability to perform well in domain-specific tasks~\cite{??}. 

%On the other hand, fine-tuning can skip prefilling the long input, because the knowledge has already been embedded in the model weights and thus the input text can be short.
On the other hand, fine-tuning embeds the knowledge inside the model, which enables it to take in a short question without the knowledge and thus skip the long prefill.
As a result, it achieves better efficiency compared to in-context learning.
However, fine-tuning suffers from bad modularity.
%First, putting all knowledge into one model dilutes its ability to perform well in domain-specific tasks~\cite{ling2024domainspecializationkeymake, chen2020recalllearnfinetuningdeep}, and in the meantime, service providers cannot control the knowledge used to generate the answer.
First, service providers cannot specify which knowledge would be used to generate the answer.
Moreover, fine-tuning needs to happen for every new knowledge and model, which may take hours to days to complete.

%The second dimension is response delay, which is defined by the time it takes from LLM receiving the user's input to the generation of the first token.
%In-context learning increases the response delay, because it needs to {\em prefill} the longer input text with knowledge before generating the first token.
%In the prefill phase, the LLM takes in the input tokens, runs the attention operation, and gets the KV cache tensor for future token generation.
%In all mainstream LLMs, the time for attention operation grows superlinearly with the input length.
%In practice, the overhead of prefilling a 12-page paper is XXX seconds when using XXX model.
%Fine-tuning has already embedded the knowledge in the model weights, so it only needs a short input and can avoid the overhead of prefilling long texts.

%In short, Figure~\ref{??} compares in-context learning and fine-tuning from the system perspective. In-context learning is more modular but sacrifices the response delay, while fine-tuning, as a non-modular design, can generate the response with a lower delay. \yh{add a few words about cost}

In short, as shown in Figure~\ref{fig:comparison}, in-context learning is more modular but sacrifices efficiency, while fine-tuning, though achieving better efficiency, suffers from the overhead of incorporating and controlling the knowledge due to bad modularity.

==> kdn.tex <==
\section{Managing knowledge with knowledge delivery networks}

\jc{we need to put a diagram of KDN here.}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/placeholder-kdn.pdf}
    \tightcaption{Placeholder diagram of KDN}
    \label{fig:kdn}
\end{figure}

% Some solutions started to use KV cache
Rather than fine-tuning and in-context learning, some recent research has started focusing on {\em KV-cache learning}, which uses KV cache as a medium of knowledge and puts it as part of the LLM input.
KV cache is a tensor generated during the prefill phase of the in-context learning, and it contains the information from the input knowledge for LLM to utilize later during text generation.
And, once generated, the KV cache can be reused in all the subsequent inference requests that require the corresponding knowledge.

% Into to KV cache: both modular and fast
By embracing KV caches, KV-cache learning is as modular as in-context learning, because swapping knowledge only requires the change of the KV cache, without touching other parts of the system.
Also, when the KV cache is in GPU, LLM can skip prefilling the long text and start generating tokens immediately, meaning that the performance (runtime cost and response delay) will be similar to fine-tuning. 
Therefore, KV-cache learning has the potential to surpass in-context learning and fine-tuning on all three dimensions as shown in Figure~\ref{fig:comparison}.
%\yh{Talk about cost reduction}

% However, using KV cache has some practical challenges
% - size is huge, and cannot fit to GPU, and on-demand loading KV is slow
% - only work for prefix, limiting the modularity 
However, KV-cache learning still faces some practical challenges.
First, the KV cache has a huge memory footprint~\cite{??}. 
For instance, the KV cache from XXX model for a 12-page paper (XXX tokens) is XXX GB.
Either GPU or CPU memory is not enough to hold the KV cache of all knowledge used for a modern LLM service~\cite{??}.
A workaround is to store KV cache in external devices like local disks or storage servers~\cite{??}.
That said, the overhead of loading the KV cache into GPU could drastically increase the response delay similar to in-context learning~\cite{??}.

%Second, the KV cache can only be reused when its corresponding text is reused as the {\em prefix} of another LLM input~\cite{??}, which makes KV-learning impractical in real-world use cases.
%For instance, retrieval augmented generation (RAG), a popular LLM application, often prepends multiple text chunks in the input to provide different knowledge necessary for answering the user query.
%In this case, $N$ text chunks may have $N!$ different ways of ordering, requiring $N!$ different KV cache tensors which are impossible to store in practice.
Second, unlike in-context learning that can incorporate different knowledge by concatenating the text chunks, different KV caches cannot be directly concatenated together.
This is because direct concatenation {\em ignores the cross-attention (\ie the relationship among different knowledge)} between different KV caches, leading to incorrect responses.
This problem limits the use of KV cache learning in popular LLM applications like RAG (retrieval augmented generation)~\cite{??}.


% Recent research help address those challenges
Recently, there have been a few works trying to address those challenges. 
Different methods have been invented to reduce the memory footprint of the KV cache, including token selection~\cite{llmlingua, h2o}, MLA~\cite{mla}, and KV cache compression~\cite{cachegen}.
Another work~\cite{cacheblend} is proposed to address the second challenge by dynamically computing the cross-attentions between the KV caches.

% Based on those, we propose the KDN
Based on those techniques, we propose the {\em knowledge delivery network} (KDN), as shown in Figure~\cite{??}.
The system has three main components:
\begin{itemize}
    \item {\em KV cache store} manages the compressed KV caches keyed by the text of each piece of knowledge.
    \item {\em KV cache delivery} quickly transmits the compressed KV cache to GPUs.
    \item {\em KV cache blender} merges multiple KV caches by computing the missed cross-attention.
\end{itemize}

LLMs can generate KV caches for different knowledge and put them into KDN online or offline.
When an inference request comes, the operator will specify which knowledge should be used, and query the KDN for the KV caches.
The KDN will retrieve the multiple KV caches corresponding to the pieces of knowledge from the KV cache store and deliver them to GPUs by KV cache delivery.
The KV caches will then be merged by the KV cache blender before input into LLM.

% Show some results
Figure~\ref{??} shows that KDN can reduce the response delay compared to in-context learning.

% Discussion
\section{Discussion}

\mypara{KDN and generation quality} 
It is generally believed that changing the KV cache, such as quantization and compression, will degrade the generation quality of LLMs.
That said, it is possible to get a KV cache with higher quality, by using a larger LLM  to tell what is the relashionship between tokens, and adjust the KV cache generated by small model correspondingly.

Our initial experiment shows that, on
\yh{Attention steering}

\mypara{Interface between KDN and LLM serving engines}
Existing production-level LLM serving engines, such as vLLM and LMDeploy, can only take the text as the input. As a result, we need to open up a KV cache communication API in these engines for these engines to take in KV cache. 

The key difficulty to implement this API is to incentivise these engines to implement this API that seems to only for KDN's sake. On this front, we argue that, this API can provide immediate values. For example, this API allows one to implement disaggregated prefilling.





==> kdn_v2.tex <==
\section{Managing knowledge with knowledge delivery networks}
\label{sec:kdn}

\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figs/placeholder-kdn.pdf}
    \vspace{-4pt}
    \tightcaption{Architecture of a Knowledge Delivery Network (KDN).}
    \label{fig:kdn}
\end{figure}

% Some solutions started to use KV cache
Rather than fine-tuning and in-context learning, some recent research has started focusing on {\em KV-cache learning}, which uses KV cache as a medium of knowledge and puts it as part of the LLM input.
KV cache is a tensor generated during the prefill phase of the in-context learning, and it contains the information from the input knowledge for LLM to utilize later during text generation.
Once generated, the KV cache can be reused in all the subsequent requests that require the corresponding knowledge.

% Into to KV cache: both modular and fast
%By embracing KV caches, KV-cache learning is as modular as in-context learning, because the KV cache is associated with each text knowledge.
Similar to in-context learning, KV-cache learning has good modularity since it also separates the knowledge and the model weights.
In the meantime, LLM can skip prefilling and start generating tokens immediately if the KV cache is on the GPU, meaning that the efficiency (runtime cost and response delay) will be similar to fine-tuning. 
Therefore, KV-cache learning has the potential to surpass in-context learning and fine-tuning on both modularity and efficiency. % as shown in Figure~\ref{fig:comparison}.
%\yh{Talk about cost reduction}

\begin{table*}[ht!]
\begin{tabular}{c|c|cc}
\hline
                                                                     & \textbf{Modularity}          & \multicolumn{2}{c}{\textbf{Efficiency}}                                              \\ \hline
                                                                     & Time to inject new knowledge & \multicolumn{1}{c|}{Inference cost (\$) per request} & Response delay (s) per request \\ \hline\hline
Fine-tuning                                                          & 10 hours                     & \multicolumn{1}{c|}{0.0052}                      & 2.63                           \\ \hline
In-context learning                                                  & 0                            & \multicolumn{1}{c|}{0.0149}                      & 10.91                           \\ \hline
% \begin{tabular}[c]{@{}c@{}}KV-cache learning\\ with KDN\end{tabular} & 0.25 hours                   & \multicolumn{1}{c|}{0.0052}                      & 2.64                           \\ \hline
\rowcolor{LightCyan}KV-cache learning w/ KDN & 0.25 hours                   & \multicolumn{1}{c|}{0.0059}                      & 2.97                           \\ \hline
\end{tabular}
\vspace{16pt}
\tightcaption{Comparison between different knowledge-injection methods under a RAG setup. With KDN, KV-cache learning is $40\times$ faster when incorporating new knowledge than fine-tuning, and achieves $3.7\times$ faster and $2.5\times$ cheaper during inference compared to in-context learning.}
\vspace{-8pt}
\label{tab:comparison}
\end{table*}


%That said, KV caches have large memory footprints, making it hard to put all knowledge in GPU or CPU memory~\cite{ragcache, yao2024cacheblend, qin2024mooncake}.
That said, it is impossible to put KV caches of all the knowledge in GPU or CPU memory due to their large memory footprint~\cite{ragcache,yao2024cacheblend,qin2024mooncake}. 
%have large memory footprints, making it hard to put all knowledge in GPU or CPU memory~\cite{ragcache, yao2024cacheblend, qin2024mooncake}.
To address this issue, we propose a new system architecture, {\em knowledge delivery network} (KDN), that stores, transmits, and composes the knowledge in the form of KV caches on demand.
Figure~\ref{fig:kdn} shows the architecture of KDN, which consists of three main components:
\begin{itemize}
    \item {\em KV cache store} manages the compressed KV caches keyed by the text of each piece of knowledge.
    \item {\em KV cache delivery} transmits the compressed KV cache to GPUs that host the LLMs.
    \item {\em KV cache blender} composes multiple KV caches corresponding to different pieces of knowledge.
\end{itemize}

% Introduce the workflow
KV caches, generated from LLMs, can be put into KDN online or offline.
When an inference request comes, the LLM sends requests to the KDN for some specific knowledge. %for the KV caches of to KDN based on the required knowledge.
The KDN then retrieves multiple KV caches corresponding to the pieces of knowledge from the KV cache store and delivers them to GPUs by the KV cache delivery.
Finally, the KV cache blender merges the retrieved KV caches and puts the composed KV cache into the LLM.
%The KV caches will then be merged by the KV cache blender before input into LLM.

%\item however, today's systems store kv caches only in gpus. assumption: storing more kv cache on other devices is too expensive and slow
%However, today's LLM serving systems, such as vLLM~\cite{kwon2023vllm}, TGI~\cite{huggingface_tgi_2024}, and SGLang~\cite{sglang}, only store a limited number of KV caches in GPUs or CPUs.
%There are two main reasons hindering the adoption of KDN: 
However, to our best knowledge, KDN does not exist in today's LLM serving engines~\cite{kwon2023vllm, sglang, huggingface_tgi_2024} due to the following two main reasons:
\textit{(i)} storing KV caches outside GPU or CPU memory is too expensive and slow due to the large size of the KV cache, and 
\textit{(ii)} composing different knowledge represented by KV caches is non-trivial because the KV cache of a text chunk can only be reused when the text is reused as the {\em prefix} in the LLM's input. %, making it hard to compose different knowledge represented by KV caches. %limiting the composability of the KV caches. 
%\textit{(ii)} the KV cache of a text chunk can only be reused when the text is reused as the {\em prefix} in the LLM's input, making it hard to compose different knowledge represented by KV caches. %limiting the composability of the KV caches. 

%Nevertheless, some emerging research helps address the above problems and enables KDN.
Nevertheless, the above problems can be addressed by some emerging research works, and thus making KDN practical.

KV cache compression techniques make it possible to cheaply store and quickly load KV caches outside GPU and CPU memory.
%The first issue can be addressed by KV cache compression techniques.
LLMLingua~\cite{jiang2023llmlingua} introduces a smaller language model to identify and remove non-essential tokens in the knowledge's text, thus reducing the size of the corresponding KV cache. %, and thus can reduce the size of the corresponding KV cache by 3-6$\times$.
H2O~\cite{zhang2023h2o} directly removes elements in the KV cache based on their importance which is calculated during the inference. %reduces the size of the KV cache by selectively evicting tokens with low attention scores.
CacheGen~\cite{cachegen} compresses the KV cache by quantizing and then encoding it into binary strings.
By combining the above techniques, the memory footprint of the KV cache can be reduced by more than 10$\times$, drastically improving the loading speed and the storage cost of the KV cache.

%There are also some works improving the composability of the KV caches.
Some recent works also improve the composability of the KV caches.
PromptCache~\cite{gim2023prompt} lets users define a prompt template with different segments, which allows each segment's KV cache to be reused at different positions rather than prefix-only.
CacheBlend~\cite{yao2024cacheblend} enables arbitrarily composing different KV caches by recomputing the cross-attention between KV caches, where the recomputation only needs 10\% computation of prefilling the full text.






Based on these techniques, we implemented LMCache (\url{https://github.com/LMCache/LMCache}), a prototype of KDN.
To compare KV-cache learning with KDN to fine-tuning and in-context learning, we measure the modularity and efficiency under a RAG use case with the following setup:
\begin{itemize}
    \item Total size of knowledge (in text): 2 million tokens.
    \item Each request: 8K tokens knowledge plus 2K tokens user chatting history\footnote{We assume the chatting history cannot be pre-learned by fine-tuning.}.
    \item Language model: Llama 3.1 70B~\cite{dubey2024llama}.
    \item Hardware: 2 Nvidia A40 GPUs.
\end{itemize}
Modularity is measured by the time\footnote{The time for fine-tuning the model is estimated from Llama-Adapter~\cite{zhang2023llamaadapter}.} of injecting the knowledge base into LLM, and efficiency is measured by inference cost\footnote{The inference cost is calculated based on the AWS cloud price~\cite{awsec2pricing}.} and response delay per request.
Table~\ref{tab:comparison} shows that with the KDN, KV-cache learning can be 40$\times$ faster than fine-tuning when injecting new knowledge, and it also achieves $3.7\times$ cheaper and 2.5$\times$ faster during inference time compared to in-context learning.

%\item recent research may upend this assumption and enable KDN

% However, using KV cache has some practical challenges
% - size is huge, and cannot fit to GPU, and on-demand loading KV is slow
% - only work for prefix, limiting the modularity 
%However, KV-cache learning still faces some practical challenges.
%First, the KV cache has a huge memory footprint~\cite{??}. 
%For instance, the KV cache from XXX model for a 12-page paper (XXX tokens) is XXX GB.
%Either GPU or CPU memory is inadequate to hold the KV cache of all knowledge used for a modern LLM service~\cite{??}.
%A workaround is to store the KV cache in external devices like local disks or storage servers~\cite{??}.
%That said, the overhead of loading the KV cache into GPU could drastically increase the response delay similar to in-context learning~\cite{??}.

%Second, the KV cache can only be reused when its corresponding text is reused as the {\em prefix} of another LLM input~\cite{??}, which makes KV-learning impractical in real-world use cases.
%For instance, retrieval augmented generation (RAG), a popular LLM application, often prepends multiple text chunks in the input to provide different knowledge necessary for answering the user query.
%In this case, $N$ text chunks may have $N!$ different ways of ordering, requiring $N!$ different KV cache tensors which are impossible to store in practice.
%Second, unlike in-context learning that can incorporate different knowledge by concatenating the text chunks, different KV caches cannot be directly concatenated together.
%This is because direct concatenation {\em ignores the cross-attention (\ie the relationship among different knowledge)} between different KV caches, leading to incorrect responses.
%This problem limits the use of KV cache learning in popular LLM applications like RAG (retrieval augmented generation)~\cite{??}.


% Recent research help address those challenges
%Recently, there have been a few works trying to address those challenges. 
%Different methods have been invented to reduce the memory footprint of the KV cache, including token selection~\cite{llmlingua, h2o}, MLA~\cite{mla}, and KV cache compression~\cite{cachegen}.
%Another work~\cite{cacheblend} is proposed to address the second challenge by dynamically computing the cross-attentions between the KV caches.
%
%% Based on those, we propose the KDN
%%Based on those techniques, we propose the {\em knowledge delivery network} (KDN), as shown in Figure~\cite{??}.
%
%
%% Show some results
%Figure~\ref{??} shows that KDN can reduce the response delay compared to in-context learning.
%
%% Discussion

\section{Missing pieces?}


\mypara{Unifying interface with LLM serving engines}
Currently, most LLM serving engines, such as vLLM~\cite{kwon2023vllm}, HuggingFace TGI~\cite{huggingface_tgi_2024}, and SGLang~\cite{sglang}, do not readily support the injection of externally provided KV caches as part of the LLM input. 
Instead, their internal implementation KV-cache management (\eg paged memory in vLLM) is deeply cobbled with the model inference implementation. 
One way to deploy KDN is to augment each LLM engine with a KDN as part of the LLM engine. 
However, as elaborated in \S\ref{sec:kdn}, developing a performant KDN is a substantial understanding, so it will cause much redundant engineering effort if each LLM engine maintains and evolves its own KDNs. 
To prevent reinventing the wheel, the LLM serving engines could interface with a separate, shared KDN provider, via two APIs:
% As a result, we need to open up a KV cache communication interface in these engines for them to interact with KDN.
% At a high level, the interface should support two operations: 
\textit{(i)} the LLM {\em stores} the KV cache with the associated text to KDN, and
\textit{(ii)} the LLM {\em retrieves} the KV cache from KDN using some text. 
Exposing these APIs is feasible, given most popular LLM engines are open-source.
Still, several design questions remain.
How to leverage heterogeneous links, such as NVLink, RDMA, or PCIe, to transfer KV caches?
% How to pipeline KV transmission with LLM inference?
Can the APIs be shared with other LLM functions, like disaggregated prefilling?

% \mypara{KDN and generation quality} 
%\jiayi{Do we need to cite anything here?}
\mypara{Improving inference quality by offline KV-cache editing}
So far, a KDN is seen as merely a passive storage facility of KV caches. 
However, by separating KV-cache management from the LLM-serving engines, KDNs open up new possibilities to improve inference quality.
Recent works have shown that if the attention matrix of an LLM input is appropriately modified, the inference quality can significantly improve~\cite{zhang2023tell, anonymous2024model}.
In other words, when a KV cache is ``deposited'' to KDN, KDN not only stores it but also can actively influence the LLM inference quality by offline editing the KV cache and returning the edited KV cache when it is retrieved next time, all of which is done {\em without any change to the model itself or the prompt input}.
% It is generally believed that changing the KV cache, such as quantization and compression, will degrade the generation quality of LLMs.
% That said, better generation quality is achievable with careful management of the input KV caches. %\jiayi{the last two sentences are contradicting?}
A possible technique is to use a larger LLM to tell the relationship between tokens and adjust the KV cache generated by a small model correspondingly. 
% However, currently, it is difficult for service providers to perform such optimizations since state-of-the-art serving engines do not provide global management of KV caches.
% KDN, in the meantime, provides a good opportunity for such optimizations, as it has centralized management of KV caches.
% We believe KDN can not only improve the performance of LLMs from the system perspective but also enable more solutions to improve the generation quality of LLMs.

We hope this paper can inspire more research to tackle the aforementioned problems.

%The key difficulty to implement this API is to incentivise these engines to implement this API that seems to only for KDN's sake. On this front, we argue that, this API can provide immediate values. For example, this API allows one to implement disaggregated prefilling.






==> motivation_v1.tex <==



\vspace{-8pt}
\section{Background and Motivation}

%\item classic ml: everything in training data. but rapid growth of usage => more knowledge than in training data is needed. 



Traditionally, machine learning models, such as computer vision~\cite{resnet,efficientdet,llava,ssd} and image generation~\cite{gan,stable-diffusion,sora}, learn all the knowledge from the training data.
However, the rapidly growing usage of large language models (LLMs) requires the ability to inject new knowledge (unseen in training) into LLM inference.
%\item examples are abundant: personal data, corporate internal docs, new internet data, (RAG) etc
For instance, chatbots~\cite{chatbot-arena,chatgpt,characterai} use a user's chatting histories as the knowledge to generate personalized responses; 
enterprises use LLM agents to answer queries based on their internal databases using retrieval-augmented generation (RAG)~\cite{rag1,rag2,rag3,factual-llm1,factual-llm2}; 
and searching engines use LLM to read fresh and relevant web data fetched from the internet for each user query~\cite{perplexity,google-enterprise,concensus}.

Recent studies have suggested that providing more contextual data is among the most efficient ways to boost the quality of LLMs in both daily and enterprise use cases~\cite{factual-llm1,factual-llm2,incontext1}.
Also, the requirements of knowledge injection grow more complex. 
For instance, in enterprise settings, AI engineers or application operators often demand the flexibility to let them directly specify which documents (or which parts of a document) should or should {\em not} be used as the context to answer a given query~\cite{Instruct69, convivablog}. 
Moreover, as new data is being collected constantly~\cite{websiteupdate, perplexityblog1}, the knowledge-injection scheme must keep up with the rapidly evolving pool of knowledge. 

While incorporating more knowledge boosts the LLM's generation quality, doing so can cause various {\em system} challenges. 
{\em In-context} learning and {\em fine-tuning} are the two popular knowledge-injection methods employed by knowledge-augmented LLM applications. % that require new knowledge. 
% In LLM applications, in-context learning and fine-tuning are two primary methods employed to incorporate new knowledge. 
Fine-tuning retrains an LLM on a new dataset using a set of labeled knowledge to update all or parts of the model's parameters.
In-context learning refers to the ability of an LLM to understand and generate responses based on the new knowledge inserted in the LLM's input text. 
Unlike fine-tuning, it leverages the existing capabilities of the model to interpret and respond to new information, without altering the model's parameters. 
% Fine-tuning adjusts the internal parameters of the model to better capture the nuances of the new knowledge in the dataset.
An alternative to in-context learning is to use the LLM to pre-compute the {\em KV cache}\footnote{KV cache is the intermediate state when LLM prefill on a text~\cite{cachegen,yao2024cacheblend,scissorhands}, which represents the LLM's understanding of the knowledge.} of the new-knowledge text so that when this knowledge is needed to supplement an LLM inference, the KV cache, instead of the text of the knowledge, can be used directly by the LLM to generate the response based on the new knowledge. 
% also puts the new knowledge as a part of the LLM input, but in the form of {\em KV cache} rather than input tokens.
This method, which we refer to as {\em KV-cache learning}, is gaining attention in large-scale LLM services. 
As we elaborate shortly, it could be a more efficient alternative to in-context learning.


%\yh{need to elaborate the scope of the discussion: In some cases, fine-tuning is needed, but the need to get new knowledge is unavoidable}
%Examples of both in-context learning and fine-tuning are abundant. 
%For instance, in-context learning is used when an LLM is given a few text segments that contain useful background knowledge (\eg several sentences demonstrating a particular style or topic) to generate appropriate responses. 
%This method is useful for applications requiring immediate adaptation to specific contexts, such as customer service chatbots or creative writing aids. 
%Fine-tuning, on the other hand, retrains a model on a specialized dataset to enhance its performance in a specific domain, like medical diagnosis or legal document analysis. 

% An emerging knowledge-injection method, known as {\em KV-cache learning}~\cite{??} \kt{For me, KV cache is not a way to inject knowledge. It's a way to save cost. Knowledge-injection-capability wise it is the same as in-context leraning...}, is getting popularity these days.


%%\item llms support three ways of incorporating new knowledge: fine-tuning (\ie in model weights), in-context learning (\ie in text), kv-cache learning (\ie in kv cache).
%To incorporate new knowledge into LLMs, existing solutions fall into three categories.
%First, {\em fine-tuning} allows developers to update a fraction of the pre-trained LLM weights with a new corpus of labeled data, so the new knowledge is embedded in the LLM weights.
%Second, {\em in-context learning} allows developers to put a piece of new knowledge (\eg a new book or report) as part of the LLM input tokens so that an LLM, without changing its weights, can learn it during the prefill phase. 
%%The first solution is fine-tuning, which embeds the new knowledge into the model weights by training the model on the knowledge.
%%The second solution is in-context learning, which puts the knowledge as part of the text input to the model.
%Finally, similar to in-context learning, {\em KV-cache learning} also puts the new knowledge as a part of the LLM input, but in the form of {\em KV cache} rather than input tokens.
%KV cache is the intermediate state when running LLM inference on the knowledge text~\cite{??}, which at a high level, represents the LLM's understanding of the knowledge. 

\begin{figure}[t!]
    \centering
    \vspace{16pt}
    %\hspace*{-0.35cm}\includegraphics[width=1.92\columnwidth]{figs/comparison-v2.pdf}
    \includegraphics[width=0.99\columnwidth]{figs/comparison-table.pdf}
    \vspace{8pt}
    \tightcaption{Different knowledge-injection methods make trade-offs between {\bf modularity} and {\bf efficiency}. With Knowledge Delivery Networks (KDNs), KV-cache learning can improve on both dimensions compared to in-context learning and fine-tuning.
    %\jc{remember to change "Performance" to "efficiency", and "KV-cache learning" to "KV-cache learning (with Knowledge Delivery Networks)"}
    }
    \label{fig:comparison}
    % \vspace{-4pt}
\end{figure}

%\item this paper takes a stab at ``how to manage knowledge for llms.'' (this is different from using llms to manage knowledge, which has a lot of recent work. this distinction needs some handholding!)
These knowledge-injection methods, particularly in-context learning, and fine-tuning, have been intensively studied and compared~\cite{fine-vs-incontext1,fine-vs-incontext2,fine-vs-incontext3} in the machine-learning communities, with a primary focus on their impact on generation quality (\eg accuracy or F1 score).
Studies have shown that both in-context learning and fine-tuning can achieve high text-generation quality if they are configured appropriately by machine-learning engineers~\cite{alghisi2024should, zhang2024raft, gupta2024rag}
%, with a primary focus on their impacts on text-generation quality measured by accuracy or F1 score.
% Many recent works~\cite{??,??,??} tried to find the best solution to incorporate new knowledge, but the literature so far has taken a machine-learning perspective, mainly focusing on the impact of text generation quality measured by accuracy or F1 score.
%In this paper, we aim to answer the question ``how to efficiently manage knowledge for LLMs''.

However, less is known about the tradeoffs of these methods presented to system engineers who implement and maintain the LLM infrastructure for knowledge-augmented LLM applications.
Therefore, this paper sheds light on these methods from a {\em system's perspective} (Figure~\ref{fig:comparison}). 
% In this paper, we compare these options from a system's perspective.
Specifically, we make two key arguments:

\begin{itemize}
\item {\em These knowledge-injection methods---in-context learning, fine-tuning, and KV-cache learning---mainly differ in the tradeoffs between their {\bf modularity} (ease of adding new knowledge and flexibility to specify injected knowledge) and {\bf efficiency} (in per-query cost and response delay).} (\S\ref{sec:tradeoffs})

\item {\em Compared to in-context learning and fine-tuning, KV-cache learning {\em could} improve both modularity and efficiency, if a new system component, called {\bf knowledge-delivery network (KDN)}, is in place to optimize the management of KV caches by harnessing several emerging research efforts.} (\S\ref{sec:kdn})
    % \item These knowledge-injection methods---specifically, in-context learning, fine-tuning, and KV-cache learning---mainly differ in their tradeoffs between {\em modularity} and {\em efficiency}. (\S\ref{sec:tradeoffs})
    % \item The emerging literature on KV cache optimization could enable KV-cache learning to achieve both higher modularity and higher efficiency compared to the more popular methods of in-context learning and fine-tuning. (\S\ref{sec:kdn})
    % Among them, KV-cache learning could achieve both higher modularity and higher efficiency, given the emerging literature on KV cache optimization from the machine learning and compute systems communities. %~\cite{cachegen, cacheblend}.
\end{itemize}
% \begin{quote}

% % are key dimensions to compare the solutions for LLMs to incorporate new knowledge, though they typically have a tradeoff
% \end{quote}

% \begin{quote}


% \end{quote}

We envision a KDN as a backend of LLM-processed knowledge (\ie KV caches), which can be a part of an LLM-serving system or shared across multiple LLM-serving systems. 
Contrary to the existing LLM-serving systems~\cite{kwon2023vllm, huggingface_tgi_2024, sglang}, which deeply couple KV caches with LLM engines (\ie binding KV caches with GPUs and managing KV caches inside the LLM inference), KDNs call for a clean {\bf\em separation} between KV-cache management and LLM serving engines, for better modularity and efficiency. 

We will outline the key components of a KDN, including a large storage pool of KV caches that leverages KV-cache hierarchy and KV-cache compression, a fast KV-cache streaming system to transfer KV caches between LLM serving engines, and a KV-cache blender module that dynamically puts together multiple pieces of knowledge stored in modularized KV caches. 
Using a prototype of KDN, we will show that some emerging research efforts have already provided preliminary techniques, which, if put together appropriately, can make highly efficient KDNs a reality. 

% To fully realize the potential of KV caches, we envision a {\em Knowledge Delivery Network} (KDN), a new system designed to store, manage, and distribute knowledge in the form of KV caches for LLMs, just like CDNs are for internet traffic today.
% We outline the key components of a KDN and how it could improve modularity and efficiency, in terms of both compute-storage cost and 
% We show that KDNs could greatly save delay and cost and improve modularity, compared to in-context learning or fine-tuning.


%\begin{itemize}
%\item we make two key arguments: 
%\begin{itemize}
%    \item from a system perspective, knowledge management should meet two goals: modular, cost-efficient and fast response.
%    \item among the three ways of incorporating new knowledge, kv-cache learning is more modular, more cost-efficient and faster, given the recent works on kv cache optimization.
%    % \item kv cache is a much more modular, cos-efficient, and responsive approach
%    % \item using kv cache is more manageable and cost efficient to operators without sacrificing quality, IF kv cache is stored in gpu mem
%\end{itemize}
%\item we propose knowledge-delivery network, a new system for llms designed make the benefits of kv-cache learning practical.
%
%\end{itemize}

==> motivation_v2_deprecated.tex <==
\section{Background and Motivation}

%\item classic ml: everything in training data. but rapid growth of usage => more knowledge than in training data is needed.

In classic machine learning tasks, such as computer vision~\cite{??, ??} and image generation~\cite{??,??}, the model learns all the knowledge from the training data.
However, the rapidly growing usage of large language models (LLMs) requires more knowledge than training data during inference time.
%\item examples are abundant: personal data, corporate internal docs, new internet data, (RAG) etc
For instance, chatbots~\cite{??} uses fresh chatting histories as the knowledge to generate new responses; 
companies build LLM agents based on their internal knowledge bases~\cite{??}; 
searching engines use LLM to process newly created webpages on the internet every day~\cite{perplexity,??}.

%\item llms support three ways of incorporating new knowledge: fine-tuning (\ie in model weights), in-context learning (\ie in text), kv-cache learning (\ie in kv cache).
To incorporate new knowledge into LLMs, existing solutions fall into two categories.
The first solution is in-context learning, which puts the knowledge as part of the text input to the model.
The second solution is fine-tuning, which embeds the new knowledge into the model weights.

In practice, both solutions have weaknesses. 
In-context learning drastically increases the computation due to {\em prefilling}~\cite{??} and thus has a longer response delay. 
For example, it takes \fillme seconds to prefill a 12-page paper before the LLM can generate the response.
Fine-tuning embeds the knowledge in the model and avoids the prefill, but the training process requires tens of GPUs running from hours to days~\cite{??}, and such training is needed for every new knowledge and every new model.


%\item this paper takes a stab at ``how to manage knowledge for llms.'' (this is different from using llms to manage knowledge, which has a lot of recent work. this distinction needs some handholding!)
In this paper, we aim to answer the question ``how to efficiently manage knowledge for LLMs'' from a system perspective of view.
More specifically, we make the following two key arguments:
\begin{itemize}
\item From a system perspective, knowledge management should meet two goals: modular and low-delay. \yh{low-delay is not the goal of `knowledge management'.}
\item KV cache, as an intermediate result of LLM inference, can be used as a medium of knowledge to achieve better modularity and lower-delay, given the recent works on KV cache optimizations~\cite{cachegen, cacheblend}.
\end{itemize}

To fully realize the potential of KV caches, we further propose the knowledge-delivery network (KDN), a new system designed to store, manage, and distribute knowledge in the form of KV caches for LLMs.


%\begin{itemize}
%\item we make two key arguments: 
%\begin{itemize}
%    \item from a system perspective, knowledge management should meet two goals: modular, cost-efficient and fast response.
%    \item among the three ways of incorporating new knowledge, kv-cache learning is more modular, more cost-efficient and faster, given the recent works on kv cache optimization.
%    % \item kv cache is a much more modular, cos-efficient, and responsive approach
%    % \item using kv cache is more manageable and cost efficient to operators without sacrificing quality, IF kv cache is stored in gpu mem
%\end{itemize}
%\item we propose knowledge-delivery network, a new system for llms designed make the benefits of kv-cache learning practical.
%
%\end{itemize}

==> outdated/intro_v1.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

The wide use of large language models (LLMs) introduces opportunities for new serving systems.
These systems should not only optimize individual queries (\eg vLLM, \fillme);
more importantly, they should also optimize for real-world workloads by embracing useful patterns {\em across} LLM queries from the same user, from different users, or even different applications.

%real-world wordloads leverage useful patterns {\em across} LLM queries from the same user, from different users or even different applications.


One major shift resulting from the wide use of LLMs is that LLM queries require a wide range of knowledge to provide the necessary contexts to generate high-quality answers. 
Such context knowledge can be stale or fresh, from the public domain or private database, common-sense or case-specific.
With such a wide variety of knowledge, it is no longer feasible to have all the potentially necessary knowledge in the training data (even with the whole web corpus). 
Instead, people rely mainly on two methods to incorporate knowledge not present in the foundation models' pre-training data. 
\begin{packeditemize}
\item {\em Fine-tuning} allows developers to update a fraction of pre-trained LLM with a new corpus of knowledge data.
This is commonly used when a large corpus of private or domain-specific data  (\eg medical or finance) are available at once and need to be learned by the model in order to provide good answers.
\item {\em In-context learning} allows developers to put a piece of new knowledge as part of the LLM input tokens so that an LLM, without changing its weights, can learn it during the prefill phase. 
This is commonly used when the new knowledge text can fit in the context window.
Since in-context learning does not need the extra training of the model, it is faster than fine-tuning.
\end{packeditemize}


\begin{figure}
    \centering
    \hspace*{-0.35cm}\includegraphics[width=.92\columnwidth]{figs/example-diagram.pdf}
    \tightcaption{}
    \label{fig:}
\end{figure}

There has been much recent research about the relative strengths and weaknesses regarding fine-tuning vs. in-context learning. 
However, the analysis so far has been framed mainly from a {\em machine-learning} perspective---which one yields higher generation quality (\eg accuracy or F1 score). 
This includes recent efforts (\eg~\cite{raft paper}) that attempt to combine the two into one unifying method. 
That said, the results so far are mostly mixed with little conclusive evidence that one always leads to better or worse quality~\cite{cite a bunch of papers here}.  


In this vision paper, we approach this question from a {\em systems} angle. 
We cast the question of how to incorporate knowledge into a functionality-placement problem, which we refer to as {\em knowledge placement}. 
Like other functionality placement problems (\eg layering in protocol stack, end-to-end argument, etc), we can reason about the implication of different knowledge-placement choices in terms of cost, performance, and evolvability. 

In particular, we ask the following questions:
\begin{packeditemize}
\item How does knowledge placement affect {\em operational cost}, in compute, storage, and communication?
\item How does knowledge placement affect {\em system performance}, in delay and throughput?
\item How does knowledge placement affect {\em evolvability}, in terms of how often it triggers extra overhead than model inference? 
\end{packeditemize}

Our analysis reveals that perhaps not surprisingly, the factor that determines better knowledge placement (between fine-tuning and in-context learning) is how often a piece of knowledge gets re-used after it is refreshed. 
On one hand, when a piece of knowledge is reused as the context in many queries, dubbed {\em hot} knowledge, it is more advantageous to fine-tune the model with the knowledge. 
On the other hand, if it is reused only in one or few queries, dubbed {\em cold} knowledge, in-context learning is favored. 

Inspired by this analysis, we further ask if there is still room to greatly improve knowledge placement beyond in-context learning and fine-tuning. 
Surprisingly, our analysis elucidates the need for a new module that optimizes for {\em warm} knowledge, which is a piece of knowledge that is used as context in LLM queries not as frequently as hot knowledge and not as rarely as cold knowledge. 
A typical example of warm knowledge can be the documents in a retrieval-augmented generation (RAG) pipeline that is actually used by multiple queries. 
Other examples of warm knowledge include chatting history and user-uploaded documents that are repeatedly analyzed. 

Surprisingly, for most warm knowledge, we show that compared to in-context learning and fine-tuning, it is more advantageous to {\em place knowledge in KV cache}, \ie storing and re-using the KV cache of the warm knowledge across queries that use the same warm knowledge. 
We refer to the placement of knowledge in KV cache as {\em knowledge sharing}.
Our analysis shows that, despite the large size of the KV cache, knowledge sharing could greatly save operational cost, delay, and throughput when serving warm knowledge, compared to in-context learning or fine-tuning.

Though storing KV cache is not new, our vision of a knowledge-sharing system generalizes and systematizes the use of KV cache as a design choice of knowledge placement.
First, we do not limit the sharing of the KV cache within one inference session of successive queries (\eg~\cite{sglang, etc}) or in one LLM-serving instance (\eg~\cite{vllm,ollama}).
Second, we show when KV cache as a knowledge-placement choice is more advantageous than alternatives (in-context learning and fine-tuning). 
Third, we connect our vision with recent technical advances that could address the key challenges of knowledge sharing.
In particular, recent work has made it possible to substantially reduce the size of KV caches and also enable the reuse of KV cache at arbitrary positions in an input.
Finally, we outline unique opportunities arising from the knowledge-sharing platform to better manage and share knowledge in LLM serving.






%KV cache is well-studied as a way to speed up inference, but due to its big size, current systems only store them in local memory and rarely store them for re-use across queries over a long timescale.
%However, we show that for warm knowledge, doing it makes sense as the cost for storing the KV caches is almost always lower than the cost for prefilling in in-context learning or fine-tuning.

%We use the term {\em knowledge-sharing} to refer to storing and sharing of KV caches of warm knowledge across LLM queries.
%Particularly, we show concrete analysis that shows when a piece of knowledge should be managed by a knowledge-sharing system.
%Moreover, we connect this proposal with recent technical developments that actually show promise to make such knowledge-sharing platform technically feasible.


==> outdated/intro_v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

The wide use of large language models (LLMs) introduces opportunities for new serving systems.
These systems should go beyond optimizing individual queries (\eg vLLM, \fillme) and instead, optimize for real-world workloads by embracing useful patterns {\em across} LLM queries from the same user, from different users, or even different applications.
%real-world wordloads leverage useful patterns {\em across} LLM queries from the same user, from different users or even different applications.
One major shift resulting from the wide use of LLMs is that different LLM queries require a wide range of knowledge to provide the necessary contexts to generate high-quality answers. 
The increased variety of knowledge can be stale or fresh, from the public domain or private database, common-sense or case-specific.
Thus, it is no longer feasible to have all the potentially necessary knowledge in the pre-training data of foundation models. 


%Instead,  on two methods to incorporate knowledge not present in the foundation models' pre-training data. 
To incorporate new knowledge in LLM inference, two primary methods are in-context learning and fine-tuning.
In-context learning allows developers to put a piece of new knowledge (\eg a new book or report) as part of the LLM input tokens so that an LLM, without changing its weights, can learn it during the prefill phase. 
Fine-tuning allows developers to update a fraction of pre-trained LLM with a new corpus of knowledge data. 
%This is commonly used when a large corpus of private or domain-specific data  (\eg medical or finance) are available at once and need to be learned by the model in order to provide good answers.
%This is commonly used when the new knowledge text can fit in the context window. Since in-context learning does not need the extra training of the model, it is faster than fine-tuning.

%This includes recent efforts (\eg~\cite{raft paper}) that attempt to combine the two into one unifying method. 
%That said,  that one always leads to better or worse quality~\cite{cite a bunch of papers here}.  


%\begin{packeditemize}
%\item {\em Fine-tuning} allows developers to update a fraction of pre-trained LLM with a new corpus of knowledge data.
%This is commonly used when a large corpus of private or domain-specific data  (\eg medical or finance) are available at once and need to be learned by the model in order to provide good answers.
%\item {\em In-context learning} allows developers to put a piece of new knowledge as part of the LLM input tokens so that an LLM, without changing its weights, can learn it during the prefill phase. 
%This is commonly used when the new knowledge text can fit in the context window.
%Since in-context learning does not need the extra training of the model, it is faster than fine-tuning.
%\end{packeditemize}





\begin{figure}
    \centering
    \hspace*{-0.35cm}\includegraphics[width=.92\columnwidth]{figs/example-diagram.pdf}
    \tightcaption{}
    \label{fig:}
\end{figure}


The capability of LLMs to learn knowledge from their inputs during inference (in addition to training) gives rise to a key question: 

\begin{quote}
{\em For each piece of new knowledge, where should it be placed and how should it be delivered to the LLM?}
\end{quote}

\noindent 
Much recent research has compared fine-tuning (\ie knowledge in training data) vs. in-context learning (\ie knowledge in input texts), but the literature so far has taken a {\em machine-learning} perspective, focusing mainly on their impact on text-generation quality, in terms of accuracy or F1 score. 

In this vision paper, we approach this question from a {\em system's} perspective. 
We cast the question of where to place each knowledge into a functionality-placement problem.
Like other functionality placement problems (\eg layering in protocol stack, end-to-end argument, etc), we analyze the implication of different knowledge-placement choices in terms of resource usage, performance, and evolvability. 
In particular, we ask the following questions:
\begin{itemize}
\item How does knowledge placement affect {\em operational cost}, in compute, storage, and communication?
\item How does knowledge placement affect {\em system performance}, in delay and throughput?
\item How does knowledge placement affect {\em evolvability}, in terms of how often it triggers extra overhead than model inference? 
\end{itemize}

We present a simplified analysis which reveals that perhaps not surprisingly, the better knowledge placement between fine-tuning and in-context learning is governed by how often a piece of new knowledge arrives and gets re-used.
If a piece of knowledge is reused as the context in many queries, dubbed {\em hot} knowledge, fine-tuning is the favored way of incorporating that knowledge in LLM.
If it is reused only in one or few queries, dubbed {\em cold} knowledge, in-context learning is favored. 

Yet, knowledge is often neither hot nor cold---reused multiple times but not frequently enough to merit fine-tuning. 
We call this {\em warm} knowledge.
A typical example of warm knowledge can be the documents in a retrieval-augmented generation (RAG) pipeline that is actually used by multiple queries. 
Other examples of warm knowledge include chatting history and user-uploaded documents that are repeatedly analyzed. 


What is a better knowledge placement and delivery scheme for such {\em warm} knowledge?
% that is neither cold nor hot, which we call {\em warm} knowledge?
Surprisingly, we found that {\em Knowledge Delivery Networks} (KDNs), which store and deliver knowledge in the form of {\em KV caches}, can be a surprisingly effective solution for warm knowledge, just like CDNs are for Internet traffic today.
We show that, despite the large size of the KV cache, KDNs could greatly save operational cost, delay, and throughput when serving warm knowledge, compared to in-context learning or fine-tuning.
%if there is still room to greatly improve knowledge placement beyond in-context learning and fine-tuning. 

%Surprisingly, our analysis elucidates the need for a new module that optimizes for {\em warm} knowledge, which is a piece of knowledge that is used as context in LLM queries not as frequently as hot knowledge and not as rarely as cold knowledge. 
%
%Surprisingly, for most warm knowledge, we show that compared to in-context learning and fine-tuning, it is more advantageous to {\em place knowledge in KV cache}, \ie storing and re-using the KV cache of the warm knowledge across queries that use the same warm knowledge. 
%We refer to the placement of knowledge in KV cache as {\em knowledge sharing}.
%Our analysis shows that, despite the large size of the KV cache, knowledge sharing could greatly save operational cost, delay, and throughput when serving warm knowledge, compared to in-context learning or fine-tuning.

Though storing KV cache is not new, our envisioned KDNs generalize and systematize the use of KV cache for knowledge placement and delivery.
First, KDNs do not limit the sharing of the KV cache within one inference session of successive queries (\eg~\cite{sglang, etc}) or in one LLM-serving instance (\eg~\cite{vllm,ollama}).
Second, we show {\em when} KV cache as a knowledge-placement choice is more advantageous than in-context learning and fine-tuning. 
Finally, we outline a technical roadmap that leverages recent technical advances to address key challenges facing KDNs and explore new opportunities arising from KDNs to better manage and share knowledge in LLM serving.

%recent technical advances that could address the key challenges facing knowledge sharing.
%In particular, recent work has made it possible to substantially reduce the size of KV caches and also enable the reuse of KV cache at arbitrary positions in an input.
%Finally, we outline unique opportunities arising from the knowledge-sharing platform to better manage and share knowledge in LLM serving.







==> outdated/modeling.tex <==
\section{Cost modeling}

\subsection{Basic assumptions and definitions}
Consider the following setup: queries with contexts are coming to an inference engine that connects to a storage server which will be cleared every $\RefreshPeriod$ minutes. We call $\RefreshPeriod$ as ``refresh period''.

To simplify the model, we made the following assumptions:
\begin{itemize}
    \item Each query's context will have the same length
    \item All the query's context in a refresh period can be known at the beginning of that period.
    \item The time to finetune the model is proportional to number of contexts
    \item The size-overhead of the fine-tuned model is proportional to number of contexts (e.g., each context has its own LoRA adapter)
\end{itemize}

We define the following hyper-parameters:
\begin{itemize}
    \item : the GPU price per time unit
    \item : the cost of storing a unit-sized object for $\RefreshPeriod$ time
    \item : the cost of transmitting a unit-sized object 
    \item $\ModelSize$: the size overhead of finetune a single context
    \item $\KVSize$: the size of KV cache of a single context
    \item $\TextSize$: the size of the text of a single context
    \item $\PromptTime$: the time to prefill the context on GPU
    \item $\QueryTime$: the time to prefill the query on GPU
    \item $\FinetuneTime$: the time to fine-tune the model in a single context
    \item $\Bandwidth$: the bandwidth between the storage server and the inference server
\end{itemize}

We use two key parameters to describe the workload during one refresh period:
\begin{itemize}
    \item $\ReuseRatio$: the ratio of contexts that have already been seen since the start of the current refresh period.
    \item $\NewRatio$: the ratio of contexts that have never been seen before (including the past refresh periods).
\end{itemize}
There is another situation that some contexts have come during past refresh periods, but not the current refresh period. 
Those contexts neither belong to $\ReuseRatio$ nor $\NewRatio$. 
Therefore, we have $\ReuseRatio + \NewRatio \leq 1$.

We define the following three systems:
\begin{itemize}
    \item System 1 (FT): if the context has never been seen before, the system will finetune it. When a query comes, the LLM only needs to take the query as the input without context.
    \item System 2 (IC): the LLM will always prefill both the query and the context before generating the answer.
    \item System 3: if the context's KV is not in the storage server, the system will prefill them and store the KV cache in the storage server. Otherwise, the system will load the KV cache from the storage server and only prefill the prompt.
\end{itemize}

\subsection{Cost/Performance model}

\begin{table*}[ht]
\begin{tabular}{|c|c|c|c|c|}
\hline
         & Avg GPU usage per query & Avg storage cost per query & Avg network usage /query & Delay \\ \hline
System 1 & $\NewRatio \cdot \FinetuneTime $ & $\NewRatio \cdot \ModelSize  $ & $\NewRatio \cdot \ModelSize $ & $\NewRatio \cdot \FinetuneTime $ \\ \hline
System 2 & $\PromptTime $ & 0 & $\TextSize  $ & $\PromptTime $ \\ \hline
System 3 & $(1 - \ReuseRatio) \cdot \PromptTime $ & $(1 - \ReuseRatio) \cdot \KVSize  $ & $\ReuseRatio \cdot \KVSize $ & $\ReuseRatio \cdot \PromptTime + (1 - \ReuseRatio) \cdot \frac{\KVSize}{\Bandwidth} $ \\ \hline
\end{tabular}
\caption{Summary of the cost and delay modeling}
\label{tab:model}
\end{table*}

\mypara{Compute cost}

System 1 needs to fine-tune the model for all the contexts that have never been seen before on GPU.
It also needs GPU to prefill the query.
Therefore, the compute cost is:
\begin{align}
(\NewRatio \cdot \FinetuneTime ) \cdot 
\end{align}

System 2 needs to prefill all the contexts and queries. Therefore, the compute cost is:
\begin{align}
(\PromptTime ) \cdot 
\end{align}

System 3 needs to prefill the contexts not seen since the start of the current refresh period and prefill all the queries. 
Therefore, the compute cost is:
\begin{align}
((1 - \ReuseRatio) \cdot \PromptTime ) \cdot 
\end{align}

\mypara{Storage cost}

System 1 has the additional size overhead to save the fine-tuned model for new contexts. 
Therefore, the storage cost is:
\begin{align}
\NewRatio \cdot \ModelSize \cdot 
\end{align}

System 2 does not have any storage cost since the queries and contexts will directly be sent to the inference server.

System 3 stores the KV for unseen contexts within this refresh period.
Therefore, the storage cost is:
\begin{align}
(1 - \ReuseRatio) \cdot \KVSize \cdot 
\end{align}

\mypara{Transmission cost}

System 1 transfers the fine-tuned model to the inference server, with the cost of:
\begin{align}
\NewRatio \cdot \ModelSize \cdot 
\end{align}

System 2 loads all the texts to GPU, with the cost of:
\begin{align}
\TextSize \cdot 
\end{align}

System 3 loads the KV cache when it is reusable, with the cost of:
\begin{align}
\ReuseRatio \cdot \KVSize \cdot 
\end{align}

\mypara{Delay}

Here, we compute the average delay per request during a refresh period.

System 1 needs to fine-tune the models for new contexts and prefill all queries. 
Therefore, the average delay is:
\begin{align}
\NewRatio \cdot \FinetuneTime 
\end{align}

The delay of system 2 consists of prefilling both the context and the query:
\begin{align}
\PromptTime 
\end{align}

System 3 needs to transmit the KV cache for reusable contexts and prefill all the queries. 
Therefore, the average delay is:
\begin{align}
\ReuseRatio \cdot \PromptTime + (1 - \ReuseRatio) \cdot \frac{\KVSize}{\Bandwidth} 
\end{align}



\subsection{Analysis}

\mypara{When will system 1 be best?}
\begin{align}
    \NewRatio \rightarrow 0
\end{align}
This means that system 1 will be best when no new context comes, and all the contexts are reusable (i.e., hot knowledge).

\mypara{When will system 2 be best?}
\begin{align}
    \NewRatio \gg 0 \And
    \ReuseRatio \rightarrow 0
\end{align}
This means that system 2 will be best when there are many new contexts coming and almost none of them are reusable (i.e., cold knowledge).

\mypara{When will system 3 be best?}
\begin{align}
    \NewRatio \gg 0 \And
    \ReuseRatio > \frac{1}{1 + \frac{\PromptTime\cdot}{\KVSize\cdot}} \And
    \frac{\KVSize}{\Bandwidth} < \PromptTime
\end{align}


==> outline-deprecated.tex <==
\section{Background and Motivation}

\begin{itemize}
\item classic ml: everything in training data. but rapid growth of usage => more knowledge than in training data is needed.
\item examples are abundant: personal data, corporate internal docs, new internet data, (RAG) etc
\item llms support three ways of incorporating new knowledge: fine-tuning (\ie in model weights), in-context learning (\ie in text), kv-cache learning (\ie in kv cache).
\item this paper takes a stab at ``how to manage knowledge for llms.'' (this is different from using llms to manage knowledge, which has a lot of recent work. this distinction needs some handholding!)
\item we make two key arguments: 
\begin{itemize}
    \item from a system perspective, knowledge management should meet two goals: modular, cost-efficient and fast response.
    \item among the three ways of incorporating new knowledge, kv-cache learning is more modular, more cost-efficient and faster, given the recent works on kv cache optimization.
    % \item kv cache is a much more modular, cos-efficient, and responsive approach
    % \item using kv cache is more manageable and cost efficient to operators without sacrificing quality, IF kv cache is stored in gpu mem
\end{itemize}
\item we propose knowledge-delivery network, a new system for llms designed make the benefits of kv-cache learning practical.

\end{itemize}

%The conventional thinking in machine learning is that the model should learn {\em all necessary knowledge} during training. 
%However, with the rapid rise of LLM applications, they often supplement LLM queries with new information not seen in training, as the contexts to enhance response quality.
%Examples are abundant. \jc{personal data, corporate internal docs, new internet data, (RAG) etc}
%
%LLMs allow three ways of incorporating new knowledge: 
%\begin{packeditemize}
%\item {\em Fine-tuning (FT)} retrains a fraction of pre-trained LLM weights with a new corpus of knowledge data.
%\item {\em In-context learning (IC)} putting the new knowledge in its text format as part of the LLM’s input (\eg the input prefix) so that LLM, without changing its weights, can learn it during the prefill phase
%\item {\em KV cache} is similar to IC except that the LLM has read the new knowledge text and produces the KV cache 
%\end{packeditemize}


\section{Managing Knowledge for LLMs}

\begin{itemize}
\item most work in ML regarding in-context vs fine-tuning focuses on accuracy. we view it from a system perspective. 
\item three key metrics: modular, cost efficiency, and speed (define each)
% \item a fundamental diff of in-context vs fine-tuning is the modularization of knowledge.
\item in-context learning puts knowledge in input text (\eg rag)
\begin{itemize}
    \item more modular
    \begin{itemize}
        \item allows operators to specify which knowledge to use
        \item not extra compute when new knowledge arrives
        \item potentially better quality: less confusion than putting all potentially conflicting knowledge in training data
    \end{itemize}
    \item but it has slow response and can be expensive
    \begin{itemize}
        \item prefill (long) contexts is slow
        \item prefill contexts takes critical gpu resources (hard to batch)
    \end{itemize}
\end{itemize}
\item fine-tuning puts all knowledge in model weights (no modularization)
\begin{itemize}
    \item fine-tuning is not modular
    \begin{itemize}
        \item operators cant control what knowledge is used to generate the answer
        \item fine-tuning has to happen for every new knowledge and every new model
        \item putting all knowledge in one model dilutes its ability to deeply understand and perform well in any single context/domain.
    \end{itemize}
    \item fine-tuning can be expensive
    \begin{itemize}
        \item each fine-tuning takes several hours at least (and probably a few times to make it right)
        \item add a rough computation: for an example set of knowledge, when fine-tuning is more expensive than in-context learning.
    \end{itemize}
    \item but it can be fast: no need to prefill
\end{itemize}
\item in short, in-context is more modular but sacrifices cost-efficiency and speed.
\end{itemize}

\section{Managing Knowledge with Knowledge Delivery Networks}

\begin{itemize}
\item kv cache is as modular as in-context learning: kv cache is associated with each text knowledge. 
\item kv cache can be almost as fast and as cheap as fine-tuned model, if the kv cache is stored in gpu memory
\item the problem is gpu or CPU memory is not enough
\item outline the KDN arch upfront: kv cache store, delivery to gpu, blending.
\item however, today's systems store kv caches only in gpus. assumption: storing more kv cache on other devices is too expensive and slow
\item recent research may upend this assumption and enable KDN
\begin{itemize}
    \item kv cache compression 
    \item kv cache blending
\end{itemize}
\item analytically, we show storing more kv caches reduces cost and delay (see the doc i shared earlier)
\item Discussion on further improvement
\begin{itemize}
    \item offline kv-cache engineering
    \item llm interface
\end{itemize}
\end{itemize}

% \subsection{Managing Knowledge with Knowledge Delivery Networks}

\subsection{KV cache: A promising medium for new knowledge}
\begin{itemize}
\item that said, ic has a downside: slow response and high cost, especially for repetitively used contexts. 
% when context is long and may incur a high repetitive cost for conext reused frequently
\item categorize knowledge: cold, hot, and warm
\item cost-delay tradeoff: ft for hot, ic for cold. 
\item what's for warm? kv cache (if in gpu mem). 
kv cache preserves the benefit of modularization, and strikes a better tradeoff between delay and cost when gpu mem is large enough
% \item categorize knowledge: length vs. frequency
% \item cost-delay tradeoff: ft for frequent, ic for infrequent or short
% \item what's for the rest (frequent and long)? kv cache (if in gpu mem).
\end{itemize}


%\section{A Knowledge Delivery Network for KV Cache Management}
\subsection{A Knowledge Delivery Network for KV Cache Management}
\begin{itemize}
\item but gpu or CPU mem is not large. 
\item outline the KDN arch upfront: kv cache store, delivery, blending.
\item current designs store kv caches only in gpus. assumption: storing more kv cache on other devices is too expensive and slow
\item recent research: 
\begin{itemize}
    \item kv cache compression 
    \item kv cache blending
\end{itemize}
\item analytically, we show storing more kv caches reduces cost and delay
\item Discussion
\begin{itemize}
    \item offline kv-cache engineering
    \item llm interface
\end{itemize}
\end{itemize}
